Get a Grip: Reconstructing Hand-Object Stable Grasps in Egocentric Videos

We propose the task of Hand-Object Stable Grasp Reconstruction (HO-SGR), the reconstruction of frames during which the hand is stably holding the object. We first develop the stable grasp definition based on the intuition that the in-contact area between the hand and object should remain stable. By analysing the 3D ARCTIC dataset, we identify stable grasp durations and showcase that objects in stable grasps move within a single degree of freedom (1-DoF). We thereby propose a method to jointly optimise all frames within a stable grasp, minimising object motions to a latent 1-DoF. Finally, we extend the knowledge to in-the-wild videos by labelling 2.4K clips of stable grasps. Our proposed EPIC-Grasps dataset includes 390 object instances of 9 categories, featuring stable grasps from videos of daily interactions in 141 environments. Without 3D ground truth, we use stable contact areas and 2D projection masks to assess the HO-SGR task in the wild. We evaluate relevant methods and our approach preserves significantly higher stable contact area, on both EPIC-Grasps and stable grasp sub-sequences from the ARCTIC dataset.

==> tables/epic_results_frankmocap.tex <==
\begin{tabular}{l|ccc|ccc|ccc}
\toprule
 & \multicolumn{3}{c|}{HOMan~\cite{Hasson2021TowardsVideos}} & \multicolumn{3}{c|}{Dynamic} & \multicolumn{3}{c}{1-DoF} \\
 & IOU & SCA@0.8 & SCA@0.6 & IOU & SCA@0.8 & SCA@0.6 & IOU & SCA@0.8 & SCA@0.6 \\
\midrule
bottle & 56.7 & 3.4 & 5.8 & \cellcolor{green!25}64.8 & \cellcolor{yellow!25}7.0 & \cellcolor{yellow!25}20.4 & \cellcolor{yellow!25}62.7 & \cellcolor{green!25}10.2 & \cellcolor{green!25}33.1 \\
bowl & 54.4 & 1.1 & 1.6 & \cellcolor{green!25}58.5 & \cellcolor{yellow!25}7.6 & \cellcolor{yellow!25}12.4 & \cellcolor{yellow!25}57.2 & \cellcolor{green!25}12.2 & \cellcolor{green!25}22.2 \\
can & 48.3 & 3.4 & 5.1 & \cellcolor{green!25}52.4 & \cellcolor{yellow!25}10.1 & \cellcolor{yellow!25}15.4 & \cellcolor{yellow!25}52.4 & \cellcolor{green!25}12.7 & \cellcolor{green!25}24.6 \\
cup & 56.9 & 5.5 & 7.8 & \cellcolor{green!25}61.4 & \cellcolor{yellow!25}6.0 & \cellcolor{yellow!25}24.2 & \cellcolor{yellow!25}60.3 & \cellcolor{green!25}10.1 & \cellcolor{green!25}36.8 \\
glass & 55.4 & 3.0 & 4.2 & \cellcolor{green!25}60.2 & \cellcolor{yellow!25}8.2 & \cellcolor{yellow!25}21.7 & \cellcolor{yellow!25}57.5 & \cellcolor{green!25}10.2 & \cellcolor{green!25}29.7 \\
mug & \cellcolor{yellow!25}59.4 & 3.9 & 6.6 & 59.0 & \cellcolor{yellow!25}5.0 & \cellcolor{yellow!25}18.0 & \cellcolor{green!25}60.1 & \cellcolor{green!25}6.7 & \cellcolor{green!25}28.7 \\
pan & \cellcolor{green!25}48.4 & 0.5 & 1.9 & 47.0 & \cellcolor{yellow!25}2.5 & \cellcolor{yellow!25}6.9 & \cellcolor{yellow!25}47.5 & \cellcolor{green!25}4.4 & \cellcolor{green!25}13.5 \\
plate & 61.1 & 1.0 & 1.6 & \cellcolor{green!25}67.1 & \cellcolor{yellow!25}12.9 & \cellcolor{yellow!25}19.3 & \cellcolor{yellow!25}66.6 & \cellcolor{green!25}18.7 & \cellcolor{green!25}30.3 \\
saucepan & 51.1 & 0.4 & 2.4 & \cellcolor{green!25}57.2 & \cellcolor{yellow!25}3.4 & \cellcolor{yellow!25}11.5 & \cellcolor{yellow!25}55.9 & \cellcolor{green!25}9.0 & \cellcolor{green!25}19.7 \\
\hline
All & 54.9 & 1.9 & 3.3 & \cellcolor{green!25}\textbf{58.6} & \cellcolor{yellow!25}7.2 & \cellcolor{yellow!25}15.5 & \cellcolor{yellow!25}57.8 & \cellcolor{green!25}\textbf{10.8} & \cellcolor{green!25}\textbf{25.2} \\
\bottomrule
\end{tabular}
